Out-of-distribution Object Detection through Bayesian Uncertainty Estimation

The superior performance of object detectors is often established under the condition that the test samples are in the same distribution as the training data. However, in many practical applications, out-of-distribution (OOD) instances are inevitable and usually lead to uncertainty in the results. In this paper, we propose a novel, intuitive, and scalable probabilistic object detection method for OOD detection. Unlike other uncertainty-modeling methods that either require huge computational costs to infer the weight distributions or rely on model training through synthetic outlier data, our method is able to distinguish between in-distribution (ID) data and OOD data via weight parameter sampling from proposed Gaussian distributions based on pre-trained networks. We demonstrate that our Bayesian object detector can achieve satisfactory OOD identification performance by reducing the FPR95 score by up to 8.19% and increasing the AUROC score by up to 13.94% when trained on BDD100k and VOC datasets as the ID datasets and evaluated on COCO2017 dataset as the OOD dataset.

==> tables/041_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[!htpb] 
% \centering
% \caption{Main results}\label{tab:main_results}
% \resizebox{1\textwidth}{!}
% \begin{tabular}
% \multicolumn{3}{l|}{Method}                                                         & \multicolumn{2}{l}{ID: Berkeley DeepDrive-100k / OOD: COCO} & \multicolumn{2}{l|}{ID: PASCAL-VOC / OOD: COCO}                                       & \multirow{2}{*}{Uncertainty Type} \\ \cline{1-7}
%                                    & Backbone & \multicolumn{1}{l|}{Detection Head} & FPR95/AUROC                    & mAP(ID)                    & \begin{tabular}[c]{@{}l@{}}FPR95/\\ AUROC\end{tabular} & \multicolumn{1}{l|}{mAP(ID)} &                                   \\ \hline
% MC Dropout                         &          &                                     &                                &                            &                                                        &                              &                                   \\
% MSP                                &          & \multicolumn{1}{l|}{}               &                                &                            &                                                        & \multicolumn{1}{l|}{}        &                                   \\
% ODIN                               &          & \multicolumn{1}{l|}{}               &                                &                            &                                                        & \multicolumn{1}{l|}{}        &                                   \\
% Mahalanobis                        &          & \multicolumn{1}{l|}{}               &                                &                            &                                                        & \multicolumn{1}{l|}{}        &                                   \\
% Energy score                       &          & \multicolumn{1}{l|}{}               &                                &                            &                                                        & \multicolumn{1}{l|}{}        &                                   \\
% Gram matrices                      &          & \multicolumn{1}{l|}{}               &                                &                            &                                                        & \multicolumn{1}{l|}{}        &                                   \\
% Vitual Outliers                    &          & \multicolumn{1}{l|}{}               &                                &                            &                                                        & \multicolumn{1}{l|}{}        &                                   \\
%                                    &          & \multicolumn{1}{l|}{}               &                                &                            &                                                        & \multicolumn{1}{l|}{}        &                                   \\
% \textbf{Bayesian Layers-RetinaNet} & ResNet50 & \multicolumn{1}{l|}{standard NMS}   &                                &                            &                                                        & \multicolumn{1}{l|}{}        &                                   \\
% \textbf{BL-ResNet50 with cls+reg}  & ResNet50 & \multicolumn{1}{l|}{}               &                                &                            &                                                        & \multicolumn{1}{l|}{}        &                                   \\
% \textbf{BL-ResNet50 with VOS}      &          & \multicolumn{1}{l|}{}               &                                &                            &                                                        & \multicolumn{1}{l|}{}        &                                   \\ \hline
% \end{tabular}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

